e-basis Coefficients of Chromatic Symmetric Functions

A well-known result of Stanley's shows that given a graph $G$ with chromatic symmetric function expanded into the basis of elementary symmetric functions as $X_G = \sum c_{\lambda}e_{\lambda}$, the sum of the coefficients $c_{\lambda}$ for $\lambda$ with $\lambda_1' = k$ (equivalently those $\lambda$ with exactly $k$ parts) is equal to the number of acyclic orientations of $G$ with exactly $k$ sinks. However, more is known. The sink sequence of an acyclic orientation of $G$ is a tuple $(s_1,\dots,s_k)$ such that $s_1$ is the number of sinks of the orientation, and recursively each $s_i$ with $i > 1$ is the number of sinks remaining after deleting the sinks contributing to $s_1,\dots,s_{i-1}$. Equivalently, the sink sequence gives the number of vertices at each level of the poset induced by the acyclic orientation. A lesser-known follow-up result of Stanley's determines certain cases in which we can find a sum of $e$-basis coefficients that gives the number of acyclic orientations of $G$ with a given partial sink sequence. Of interest in its own right, this result also admits as a corollary a simple proof of the $e$-positivity of $X_G$ when the stability number of $G$ is $2$. In this paper, we prove a vertex-weighted generalization of this follow-up result, and conjecture a stronger version that admits a similar combinatorial interpretation for a much larger set of $e$-coefficient sums of chromatic symmetric functions. In particular, the conjectured formula would give a combinatorial interpretation for the sum of the coefficients $c_{\lambda}$ with prescribed values of $\lambda_1'$ and $\lambda_2'$ for any unweighted claw-free graph (not necessarily an incomparability graph, as in the setting of the Stanley-Stembridge conjecture).

==> commands.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}

\newcommand{\rndm}[1]{\def\arraystretch{0.91}\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\m}[1]{\def\arraystretch{0.91}\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\plainm}[1]{\def\arraystretch{0.91}\begin{matrix}#1\end{matrix}}
\newcommand{\arr}[2]{\def\arraystretch{0.91}\begin{array}{@{}#1@{}}#2\end{array}}

\newcommand{\lrp}[1]{\left(#1\right)}
\newcommand{\lrp}[1]{\left[#1\right]}
\newcommand{\bp}[1]{\big(#1\big)}
\newcommand{\ap}[1]{\langle #1 \rangle}
\newcommand{\bap}[1]{\big\langle #1 \big\rangle}
\newcommand{\Bb}[1]{\Big[#1\Big]}
\newcommand{\ts}[1]{{\textstyle #1}}
\newcommand{\ds}[1]{{\displaystyle #1}}
\renewcommand{\th}{^{\mathrm{th}}}
\newcommand{\fl}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\cl}[1]{\left\lceil #1 \right\rceil}

\DeclareMathOperator{\swts}{swts}
\DeclareMathOperator{\sink}{sink}
\DeclareMathOperator{\Sink}{Sink}
\DeclareMathOperator{\sgn}{sgn}


\newtheorem{lemma}{Lemma}
\newtheorem*{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}{Definition}

\linespread{1.1}

